Photon-Driven Neural Path Guiding

Although Monte Carlo path tracing is a simple and effective algorithm to synthesize photo-realistic images, it is often very slow to converge to noise-free results when involving complex global illumination. One of the most successful variance-reduction techniques is path guiding, which can learn better distributions for importance sampling to reduce pixel noise. However, previous methods require a large number of path samples to achieve reliable path guiding. We present a novel neural path guiding approach that can reconstruct high-quality sampling distributions for path guiding from a sparse set of samples, using an offline trained neural network. We leverage photons traced from light sources as the input for sampling density reconstruction, which is highly effective for challenging scenes with strong global illumination. To fully make use of our deep neural network, we partition the scene space into an adaptive hierarchical grid, in which we apply our network to reconstruct high-quality sampling distributions for any local region in the scene. This allows for highly efficient path guiding for any path bounce at any location in path tracing. We demonstrate that our photon-driven neural path guiding method can generalize well on diverse challenging testing scenes that are not seen in training. Our approach achieves significantly better rendering results of testing scenes than previous state-of-the-art path guiding methods.

==> 3-method-new.tex <==
\newcommand{\Px}{\bm{x}}
\newcommand{\DirO}{\omega_{o}}
\newcommand{\DirI}{\omega_{i}}
\newcommand{\DeltaO}{\Delta\Omega}
\newcommand{\DeltaA}{{\Delta A}}
\newcommand{\PathN}{{N_c}}
\newcommand{\PhotonN}{{N_p}}
\newcommand{\PhotonVoxelM}{{M}}
\newcommand{\PathVoxelM}{{M}}
\newcommand{\PhotonNormalVar}{{V_n}}
\newcommand{\SMap}{S}



\LinesNumbered
\begin{algorithm}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    Initialize a regular spatial grid $\mathbb{G}$\;
    \For{each iteration}
    {
    Trace $2^{k}$ SPP path samples to detect valid voxels and render intermediate result (Sec.\ref{sec:iterative})\;
    Trace $2^{k}$ batches of $\PhotonN$ photons from light sources (Sec.\ref{sec:iterative})\;
    Binning and accumulate energy $\Delta\Phi_{p}$ into raw maps $\SMap_{e}$ (Equ.\ref{eqn:photon})\;
    Spatial partitioning based on photon statistics (Sec.\ref{sec:iterative})\;
    Reconstruct sampling maps $\SMap_{d}$ using a pre-trained neural network (Sec.\ref{sec:learning})\;
    }
    Guide remaining path samples using learned $\SMap_{d}$ (Sec.\ref{sec:guiding})\;
    Combine all rendered results to final pixel color $\mathbb{I}_{\text{pix}}$\;
    \caption{Neural path guiding from progressive photons}
    \label{algo_pseudo}
\end{algorithm}

\Comment{
inspired by \cite{Rath2020}. On the sampling map, for a bin $\DeltaO_{k_i}$ that contains $N_{\DeltaO_{k_i}}$ photons, a photon with energy $\Phi_p$ has the equivalent estimated energy $\Phi_p^{\prime} = N_{\DeltaO_{k_i}} \cdot \Phi_p$ that flows through the entire solid angle $\DeltaO_{k_i}$.
Basically, instead of considering the sum of photon energies (as in Eqn.~\ref{eqn:photon}), we consider the sum of the squares of the energies; this leads to a guiding distribution that is aware of the variance of incident photon energies, since $\mathbb{E}[(\Phi_p^{\prime})^2] = \mathbb{E}^2[\Phi_p^{\prime}] + \mathbb{V}[\Phi_p^{\prime}]$ (where $\mathbb{E}$ and $\mathbb{V}$ represent expectation and variance respectively). 
The final guiding distribution is proportional to the square root of the accumulated squared energies:
\begin{equation}
    p_{\text{guide-var}}(\DirI) \propto \sqrt{\frac{1}{N_{\DeltaO_{k_i}}} \sum_{\omega_p \in \DeltaO_{k_i}} (\Phi_p^{\prime})^2} =  \sqrt{N_{\DeltaO_{k_i}} \cdot \sum_{\omega_p \in \DeltaO_{k_i}} (\Phi_p^2)}
    \label{eqn:target_var}
\end{equation}
If the variance is zero, then this formula downgrades to $p_{\text{guide}}(\DirI) \propto \sqrt{N_{\DeltaO_{k_i}}^{2}\Phi_p^2} = \sum_{\omega_p \in \DeltaO_{k_i}} \Phi_p = \Phi$ which is exactly our original target density (Equ.\ref{eqn:target}). This distribution essentially emphasize more on high-variance regions and less on low-variance regions; we show examples of such variance-aware sampling maps compared the original radiance-based sampling maps in Fig.xxxx. 
While the modification to the original Eqn.~\ref{eqn:photon} and
\ref{eqn:target} is moderate, we observe interesting better performance in many testing scenes, when using this variance-aware distribution (see Fig.xxx). Since using photons to measure the variance of radiance can be less accurate and effective than using path samples as did in \cite{Rath2020}, in most cases the improvement is consistent but relatively small.
}


\section{Neural path guiding using a hierarchical grid}
\label{sec:neuralguiding}
In this section, we introduce our novel path guiding framework that leverages our presented deep network to reconstruct high-quality sampling maps in a hierarchical grid.
Our full framework is illustrated in Fig.~\ref{fig:system}. 
We first iteratively build a hierarchical grid with per-voxel sampling maps. The sampling map in each voxel can be accessed in $O(1)$ time by its hashing index in the grid. In each iteration, we trace preliminary camera paths for detecting valid voxels, and we trace photons and accumulate photon energies. These samples are also used for adaptively partitioning the scene space to a hierarchical grid and reconstructing the sampling map for each voxel of the grid (see.~\ref{sec:iterative}).
We then do a final path tracing pass (see.~\ref{sec:guiding}), in which path sampling at every bouncing point of every traced ray can be guided with importance sampling of the reconstructed sampling maps. The final rendering result is computed from all path samples from both training and final path tracing. The entire pseudo process is illustrated in Algorithm~\ref{algo_pseudo}.

\begin{figure}[!ht]
    \includegraphics[width=\linewidth]{image/system.pdf}
    \caption{The proposed path guiding framework. We build a hierarchical grid to store per-voxel sampling maps. In each iteration, we trace camera rays and photons for spatial grid partitioning and sampling map reconstruction. Then, the learned sampling maps are used to importance sampling the remaining path samples.  }
    \label{fig:system}
\end{figure}

\subsection{Sampling map reconstruction}
\label{sec:iterative}
To enable path guiding at any 3D scene point, we adaptively construct a hierarchical grid for local sampling map reconstruction.
We start from a regular 3D grid of voxels that covers the entire bounding-box of the scene at a initial coarse resolution.
We then iteratively trace preliminary camera paths and light photons in the scene to locate valid voxels, compute the sampling maps, and sub-partition the grid.

\paragraph{Detect valid voxels to store sampling maps.} While we can compute a sampling map for every voxel in the grid for path guiding, this is usually costly and in fact unnecessary, since many voxels may not be reached by any paths in the final rendering.
Therefore, we instead only reconstruct sampling maps for voxels that are likely to be intersected in the final path tracing pass, avoiding the waste of reconstructing extra sampling maps. 
This is achieved by tracing a set of $\PathN$ camera paths in every iteration, leading to sequences of path intersection points; thereby we mark any voxels that are newly intersected by a path as valid voxels, for which sampling maps will be computed. 

\Comment{
Note that, these preliminary paths are not for final rendering but only for detecting valid voxels that will be used for guiding.}

To get a reasonable valid voxel set for sampling map reconstruction, we follow the same path sampling (as is described in Sec.~\ref{sec:guiding}) strategy in our final path tracing pass for tracing these intermediate camera paths. In other words, the tracing of each intermediate camera path can be also guided, if it intersects a voxel that already has a sampling map reconstructed in previous iterations. 

\paragraph{Tracing samples to reconstruct sampling maps.}
\Comment{
Along with valid voxel detection, the irradiance of traced path samples are accumulated to compute the irradiance map; the irradiance map records the sum of the average irradiance of all hit path samples $E_{j,k}$ (in all current and previous iterations) coming from any directions in the voxel, as is expressed by Eqn.~\ref{eqn:path}. }
In each iteration,
we trace a sparse set of $\PhotonN$ photons.
For any valid voxel (marked by any camera paths), we accumulate photon energies to compute the energy map; the energy map records the sum of the energies of all hit photons $\Phi_{j,k}$ in the voxel, as is expressed by Eqn.~\ref{eqn:photon}. The photon power is bilinearly splatted to the 4 nearest bins on the map.
The energy map will be normalized to a pair of raw sampling maps $\SMap_e$ that is sent to the network for final sampling map reconstruction.
As discussed in Sec.~\ref{sec:learning}, we also provide additional input buffers (photon count, previous raw sampling map, and binary mask) for the network. 
Specifically, we record the number of accumulated photons; we also keep the last raw sampling map and number of photons.
After tracing all photons in a iteration, we collect all valid voxels that have new photons arrived and reconstruct the sampling maps $\SMap_d$ using our deep neural network for path guiding. Similar to \cite{muller2017practical} and \cite{Rath2020}, we use the exponential sample count mechanism where we increase the number of path samples and photon batches in each iteration geometrically. Therefore, the variance of the input sampling map is roughly halved after each iteration. The final rendered result $\mathbb{I}_{\text{pix}}$ is computed from all traced path samples in both training and final path tracing.

\paragraph{Adaptive spatial partitioning.} 
It is not efficient to use a regular grid for spatial partitioning, since various local spatial regions may involve highly diverse geometry, appearance, and lighting distributions.
Therefore, we construct a hierarchical grid by iteratively subdividing the initial regular grid, where a voxel is divided to a binary tree as needed in a way that is similar to SD-tree in early $T_h$ iterations. 
Our hierarchical grid is built to adapt to the complexity of local geometry and incident light fields.
We leverage the statistics of the traced photons in each iteration for the voxel subdivision.
In particular, for each voxel, we consider $\PhotonVoxelM$ -- the total number of photons hitting the voxel in one iteration -- and $\PhotonNormalVar$ -- the variance of the surface normals at the photon hitpoints in one iteration.
A voxel is split into two sub-voxels by the middle of photon positions along a spatial axis if $\PhotonVoxelM > \PhotonVoxelM_{\text{thr}}$ or $\PhotonNormalVar > \PhotonNormalVar_{\text{thr}}$.
These simple photon statistics are easy to compute, enabling efficient subdivision; this subdivides voxels that either have complex light fields (dense photons) or complex geometry (large normal variation).
Once a voxel is subdivided, its two sub-voxels are reset with new sampling maps which have roughly half the photons. In addition, if a voxel contains less than $W_{\text{thr}}$ photons which are too sparse, we collect more samples from its one-surrounding neighboring voxels and create a new parent voxel that covers a bigger region. 
In this work, we proceed spatial partitioning in the first $T_h = 2$ iterations since the initial regular grid already had a good spatial resolution, and use $T = 6\sim12$ total iterations for path and photon tracing; thereby every subdivided voxel can have enough data for sampling map reconstruction. Besides, the sampling maps in parent voxels will be kept and to be used in case of any sub-voxel is invalid. After the spatial partitioning, the subsequent traced photons are accumulated in both parent and sub-voxels.

\begin{figure}[h]
    \includegraphics[width=\linewidth]{image/training_scenes.png}
    \caption{Example scenes used for training our proposed neural network.}
    \label{fig:scenes}
\end{figure}

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

\definecolor{aquamarine}{rgb}{0.67, 0.94, 0.82}

\begin{table*}[t]
	\begin{center}
		%\resizebox{\linewidth}{!}{
		
		\begin{tabular}{p{0.7in}|P{0.3in}P{0.4in}P{0.4in}P{0.4in}P{0.4in}P{0.4in}|P{0.3in}P{0.4in}P{0.4in}P{0.4in}P{0.4in}P{0.4in} }  
			%\multicolumn{10}{|c|}{\Scenea}\\
			\hline  %\STAB{\rotatebox[origin=c]{90}{\Scenea}}
			Scene/Method & PT & \cite{bako2019offline}  & \cite{vorba2014line}  &  \cite{muller2017practical} 
			 &  \cite{Rath2020} & \textbf{Ours} &  PT & \cite{bako2019offline}  & \cite{vorba2014line} & \cite{muller2017practical} & \cite{Rath2020} & \textbf{Ours} \\
			 \hline
			 Metric & \multicolumn{6}{c|}{rMSE $\downarrow$} & \multicolumn{6}{c}{SSIM $\uparrow$}\\
			\hline
			%\cline{2-10}
			\multirow{1}{*}{\textsc{Caustics Egg}}& 0.3187 & 0.1353  & 0.0462 & \cellcolor{yellow!50} 0.0311   & \cellcolor{orange!30} 0.0121 & \cellcolor{pink} 0.0052 & 0.1017  & 0.1824  & 0.3472  & \cellcolor{aquamarine} 0.4581 & \cellcolor{cyan!30} 0.7006 & \cellcolor{blue!30} 0.8242 \\
			\hline
			\multirow{1}{*}{\textsc{Veach Ajar}}& 0.3684 & 0.2585  & 0.0154 & \cellcolor{yellow!50} 0.0073   & \cellcolor{orange!30} 0.0047 & \cellcolor{pink} 0.0011 & 0.0474  & 0.0898   & 0.4579  & \cellcolor{aquamarine} 0.5455 & \cellcolor{cyan!30} 0.6325 & \cellcolor{blue!30} 0.8572 \\
			\hline
			\multirow{1}{*}{\textsc{Bathroom}}& 0.0610 & 0.0403  & \cellcolor{yellow!50} 0.0204  & 0.0249   & \cellcolor{orange!30} 0.0142 & \cellcolor{pink} 0.0050 & 0.4481  & 0.4725   & \cellcolor{aquamarine} 0.5472  & 0.5260 & \cellcolor{cyan!30} 0.5924 & \cellcolor{blue!30} 0.7427 \\
			\hline
			\multirow{1}{*}{\textsc{Hotel}}& 0.4176 & 0.2607 & 0.2838  & \cellcolor{yellow!50} 0.0812   & \cellcolor{orange!30} 0.0792 & \cellcolor{pink} 0.0276 & 0.0695 & 0.1155  & 0.0914  & \cellcolor{aquamarine} 0.2665 & \cellcolor{cyan!30} 0.2801 &  \cellcolor{blue!30} 0.4378 \\
			\hline
			\multirow{1}{*}{\textsc{Staircase}}& 0.0176 & 0.0183  & 0.0110 &\cellcolor{yellow!50} 0.0045   & \cellcolor{orange!30} 0.0038 &  \cellcolor{pink} 0.0013 & 0.4810  & 0.4957   & 0.6513  & \cellcolor{aquamarine} 0.7337 & \cellcolor{cyan!30} 0.8626 & \cellcolor{blue!30} 0.8951 \\
			\hline
			\multirow{1}{*}{\textsc{Living Room}}& 0.1928 & 0.1553  &  \cellcolor{orange!30} 0.0235 & 0.0468   & \cellcolor{yellow!50} 0.0416 & \cellcolor{pink} 0.0060 & 0.1360  & 0.1719 & \cellcolor{cyan!30} 0.4734  & 0.2960 & \cellcolor{aquamarine} 0.3327 & \cellcolor{blue!30} 0.6576 \\
			\hline
			\multirow{1}{*}{\textsc{Spaceship}}& 0.2212 & 0.0914  & \cellcolor{orange!30} 0.0198  & 0.0716   & \cellcolor{yellow!50} 0.0389 & \cellcolor{pink} 0.0137  & 0.5610  & 0.7476 & \cellcolor{cyan!30} 0.8611   & 0.7452 & \cellcolor{aquamarine} 0.8124 & \cellcolor{blue!30} 0.8793 \\
			\hline
			\multirow{1}{*}{\textsc{Classroom}}& 0.0733 & 0.0514  & 0.0124 & \cellcolor{yellow!50} 0.0085   & \cellcolor{orange!30} 0.0038 & \cellcolor{pink} 0.0021   & 0.2789  & 0.3037 & 0.5756   & \cellcolor{aquamarine} 0.6352 & \cellcolor{cyan!30} 0.7681 & \cellcolor{blue!30} 0.8234 \\
			\hline
			\multirow{1}{*}{\textsc{Wild Creek}}& 0.1425 & 0.1100  & \cellcolor{yellow!50} 0.0560 & 0.0618   & \cellcolor{orange!30} 0.0549 & \cellcolor{pink}  0.0382  & 0.3023  & 0.3734 & \cellcolor{aquamarine} 0.4890  & 0.4852 & \cellcolor{cyan!30} 0.5386 & \cellcolor{blue!30} 0.6222 \\
			\hline
			\multirow{1}{*}{\textsc{Torus}}& 0.0511 & 0.0425 & \cellcolor{yellow!50} 0.0150 & \cellcolor{orange!30} 0.0015   & \cellcolor{orange!30} 0.0015 & \cellcolor{pink} 0.0005  & 0.2610  & 0.6660 & 0.7864  & \cellcolor{aquamarine} 0.9150 & \cellcolor{cyan!30} 0.9300 & \cellcolor{blue!30} 0.9529 \\
			\hline
			\multirow{1}{*}{\textsc{Kitchen}}& 0.0644 & 0.0578  & 0.0249 & \cellcolor{yellow!50} 0.0063   & \cellcolor{orange!30} 0.0035 &  \cellcolor{pink} 0.0030  & 0.3898  & 0.4173  & 0.4655  & \cellcolor{aquamarine} 0.6753 & \cellcolor{cyan!30} 0.7873 & \cellcolor{blue!30} 0.8168 \\
			\hline
			\multirow{1}{*}{\textsc{Pool}}& 0.1175 & 0.0528  & 0.0026  & \cellcolor{yellow!50} 0.0025   & \cellcolor{orange!30} 0.0016 &  \cellcolor{pink} 0.0011  & 0.2264  & 0.4595 & 0.8551  &  \cellcolor{aquamarine} 0.8598 & \cellcolor{cyan!30} 0.9364 & \cellcolor{blue!30} 0.9510 \\
			\hline
		\end{tabular}
		
		%}
		\caption{Quantitative results on the full-resolution images. Red, orange, and yellow denote the best, the second best, and the third best one in terms of rMSE (lower is better). Purple, blue, and cyan denote the best, the second best, and the third best one in terms of SSIM (higher is better). }
		\vspace{-5mm}
		\label{tab:quant_rmse}
	\end{center}
\end{table*}

\subsection{Guiding path tracing}
\label{sec:guiding}
Once the hierarchical grid with per-voxel sampling maps is iteratively constructed,
we proceed a final path tracing to render the final image, guided by the reconstructed sampling maps. Each sampling map is accessed efficiently in $O(1)$ time using the hashing index in the grid. If a sub-voxel is invalid or if the photons are too sparse, the reconstructed sampling map in its parent voxel is used for guiding.
Since we only consider the incident radiance (integrated as energy) for our sampling maps, we apply a one-sample MIS similar to previous works to combine guided sampling and BSDF sampling, as discussed in Eqn.~\ref{eqn:target_mis}.

This combined sampling however requires a parameter $\alpha$ that determines how often either sample strategy is selected.
Usually, $\alpha=0.5$ is a simple choice and performs reasonably well in previous work \cite{muller2017practical}. An $\alpha$ that is learned by an online gradient descent optimizer (\cite{mueller19guiding}) is also presented for better performance, which however requires expensive online training.
We present a heuristic $\alpha$ computation, based path statistics, which is simple but effective in practice.
To do so, we apply path guiding for tracing the camera paths in the sampling map reconstruction (Sec.~\ref{sec:iterative}) and collect the contributions of the sampled paths for $\alpha$ estimation.
In particular, we initially use $\alpha=0.5$ in each voxel for guiding the iterative path tracing. 
Once a path is intersected and re-sampled in a valid voxel, we accumulate its actual path contribution $L_{i}(\Px, \DirI) \cos \theta_i f_{r}(\Px, \DirI, \DirO)$, in $\nu_{\text{BSDF}}$ and $\nu_{\text{Guide}}$, where $\nu_{\text{BSDF}}$ records the sum of all path contributions got from BSDF sampling and $\nu_{\text{BSDF}}$ records the sum of path energies from guided sampling.
Once a total number of $\PathVoxelM=50$ paths are sampled in valid voxel, we update the ratio of the accumulated path contributions from the two strategies to determine the mixing weight $\alpha$ for following path guiding (update after each iteration): 
\begin{equation}
    \begin{split}
     p(\DirI) & = \alpha p_{\text{BSDF}}(\DirI) + (1-\alpha)p_{\text{guide}}(\DirI) \\
                    & = \frac{\nu_{\text{BSDF}}}{\nu_{\text{BSDF}} + \nu_{\text{Guide}}} p_{\text{BSDF}}(\DirI) + \frac{\nu_{\text{Guide}}}{\nu_{\text{BSDF}} + \nu_{\text{Guide}}}p_{\text{guide}}(\DirI)
    \end{split}
    \label{eqn:mis_coef}
\end{equation}
This heuristic mixing weight considers the data that reflects the actual performance of BSDF sampling and guiding sampling, leading to effective one-sample MIS sampling in our path guiding.


%Here $E(\Px, \DeltaA_j)$



%Inspired by \cite{jensen1995importance}, we consider using photons to compute sampling maps that approximate the incident light at a local region.

%Recent unidirectional path tracing methods \cite{muller2017practical,Rath2020} leverage view-dependent spatial trees to partition the space and compute full spherical sampling maps to represent the directions in a 3D region.



\Comment{
In practice, path guiding relies on early path samples to approximate the incident light field $L_{i}(\Px, \DirI)$ as a guiding distribution; remaining samples are then sampled from either guiding or BSDF distribution according to Eqn.~\ref{eqn:target_mis}.


Very recently, \citet{Rath2020} observes that it is often infeasible to perfectly obtain the target density (Equ.\ref{eqn:target}) for every intersection point in practice. Thus, the variance of $L_{i}(\Px, \DirI)$ should also be considered, which leads to the square root of the second moment:
\begin{equation}
    p_{\text{guide-variance-aware}}(\DirI) \propto \sqrt{\mathbb{E}[L_{i}^{2}(\Px, \DirI)]}|\cos\theta_{i}|
    \label{eqn:target_variance}
\end{equation}
In fact, the choice between Equ.\ref{eqn:target} and Equ.\ref{eqn:target_variance} is orthogonal to our proposed framework. In this paper, we develop two versions of our system where the \textit{radiance version} uses Equ.\ref{eqn:target} and the \textit{variance version} uses Equ.\ref{eqn:target_variance} as the target density function. Integrating more advanced functions such as the \textit{full target density} proposed in \citet{Rath2020} into our system is left for future work.

In practice, however, we can only store a discrete set of $s_{i}$ where each one represents the total amount of incident radiance with respect to a finite subtended solid angle $\Delta\omega$:
\begin{equation}
    E_{i}(\Px, \Delta\omega) = \int_{\Delta\omega} L_{i}(\Px, \DirI)|\cos\theta_{i}|d\DirI
    \label{eqn:irradiance} = \frac{\Phi}{\Delta A}
\end{equation}
this is the \textit{irradiance} $E_{i}$ which indicates the amount of incident \textit{energy} $\Phi$ per unit area that flows through $\Delta\omega$. Therefore, for target density Equ.\ref{eqn:target} and Equ.\ref{eqn:target_variance}, the stored value $s_{i}$ can be written as:
\begin{equation}
    s_{i} \propto \int_{\Delta\omega} p_{\text{guide}}(\DirI)d\DirI
    \label{eqn:store_weight_target}
\end{equation}
and
\begin{equation}
    s_{i} \propto \sqrt{|\Delta\omega|\int_{\Delta\omega} p_{\text{guide-variance-aware}}^{2}(\DirI)d\DirI}
    \label{eqn:store_weight_target_variance}
\end{equation}

In some challenging light transport scenarios, it can be hard to get a good estimated $L_{i}(\Px, \DirI)$ from a small number of path samples, thus learning the target density will become slow (i.e., cold start problem). In these cases, using photons is often a better choice. Photons are particles emitted from light sources. Each photon carries a partial energy (i.e., flux) $\Delta\Phi$ of the light's power and a direction that roughly indicates where the radiance comes from \cite{jensen1995importance}. After photons leave the light source, they are bounced and distributed within the scene. When a photon hits a diffuse or glossy surface, it is stored at the intersection point on the surface. In general, the stored photons can approximately represent the incident radiance distribution at each intersection point $\Px$:
\begin{equation}
    L_{i}(\Px, \DirI | \DirI \in \Delta\omega) \approx \frac{1}{\Delta\omega \Delta A \cos\theta_{i}}\sum_{p=1}^{m}\Delta\Phi_{p} \propto \frac{1}{\Delta\omega \cos\theta_{i}}\sum_{p=1}^{m}\Delta\Phi_{p}
    \label{eqn:photonvar}
\end{equation}
where $m$ is the number of photons that come from a set of directions $\Delta\omega$ and stored in the neighboring region $\Delta A$ of $\Px$, and $\Delta\Phi_{p}$ is the energy flux carried by the photon $p$. In this work, we use photon energy to estimate $L_{i}(\Px, \DirI)$ and reconstruct the target density function (Equ.\ref{eqn:target} and Equ.\ref{eqn:target_variance}) by storing discrete $s_{i}$ values (Equ.\ref{eqn:store_weight_target} and Equ.\ref{eqn:store_weight_target_variance}) in a spatial cache. Based on our experiments (Sec.\ref{sec:eval}), our photon-driven system works well for challenging scenes with complex lightings, especially where path samples are difficult to find the light sources while photons are easily reachable. Besides, photon-driven methods can better explore the entire sampling space, while path sample based methods may get stuck in a sampling direction once a light source is found which is similar to the local exploration issue in Metropolis light transport.  




\section{Method}
\label{sec:method}

\subsection{System Overview}
\begin{figure}[!ht]
    \includegraphics[width=\linewidth]{image/system.pdf}
    \caption{We train our system iteratively to learn sampling density maps and store them in a spatial cache. In every iteration, path samples are generated from the camera, and photons are emitted from light sources. Path samples determine where to create new energy map in the scene, and energy of each photon is deposited to the nearest map in the spatial cache. These energy maps then pass through a pre-trained neural network that can reconstruct dense sampling maps which are then used for guiding remaining path samples in training and rendering. Furthermore, the spatial cache that stores the maps is updated on-the-fly through iterations.}
    \label{fig:system}
\end{figure}

The entire proposed system is summarized in Fig. \ref{fig:system}. We first learn target sampling densities $p(\DirI)$ at different locations in the scene through iterative training. After the training is completed, we use the learned densities to guide path samples in both the remaining training and rendering. At the beginning, the scene is partitioned into many small voxels using a fixed-resolution 3D hash grid. These voxels are used for caching the learned densities at different locations (Sec.\ref{sec:cache}). Here, we use 2D images to store $s_{i}$
and density values, where each bin/pixel ($i$, $j$) represents a subset of incident directions $\{ \DirI | \DirI \in \Delta\omega \}$ over a sphere. We will call these stored images as \textit{maps} in the rest of this paper.

During training, we trace path samples and adaptively initialize the maps. For every intersection point, if a map does not exist in the voxel that contains the point, an empty map $\SMap_{e}$ is created and cached in the voxel. Next, photons are emitted from the light sources. Since photons can represent the incident radiance field (Equ.\ref{eqn:photon}), we reconstruct $L_{i}(\Px, \DirI)$ from neighboring photons at each intersection point $\Px$ by mapping each photon's direction to a 2D position on $\SMap_{e}$ and splatting its energy $\Delta\Phi$ to $\SMap_{e}$ (Sec.\ref{sec:cache}). In other words, every bin on $\SMap_{e}$ stores the $s_{i}$ value in Equ.\ref{eqn:store_weight_target} or Equ.\ref{eqn:store_weight_target_variance} representing the incident energy that flows through the bin. After the energy is consumed by the map, the photon is deleted from the memory.

We observe that $M_{e}$ is usually quite noisy since photons are discrete samples of light power. Therefore, we train a neural network that takes these noisy maps as inputs and reconstructs the dense and smooth sampling maps $M_{d}$ (Sec.\ref{sec:neural}). The network is trained on offline data using either Equ.\ref{eqn:target} or Equ.\ref{eqn:target_variance} as the ground-truth output. This neural network reconstruction is only executed to update $M_{d}$ when enough amount of new photon energy is consumed into $M_{e}$ after every several new iterations. Since $M_{e}$ gets continuously improved over iterations by consuming more photons, the latest reconstructed $M_{d}$ also gets better over time. After reconstruction, $M_{d}$ are stored in the voxels and used to guide remaining path samples by allowing intersection points to reuse the cached density maps $M_{d}$ for importance sampling. 

Thanks to our spatial hash grid, each voxel can be accessed by its index in $O(1)$ time. Therefore, depositing photon energy and searching nearest density map $M_{d}$ are faster on our hash grid than on tree structures. Furthermore, we adaptively subdivide the voxels into smaller ones based on the collected photon statistics to allow different caching granularity at different parts of the scene, which can be seen as the combination of the hash grid and the hierarchical tree (Sec.\ref{sec:cache}). 

After training is completed, the learned density maps $M_{d}$ are used to guide path samples in rendering. For each intersection point, the reflected ray is importance sampled from the nearest cached $M_{d}$. Since the reconstructed density maps can contain zeros, we combine the guiding sampling with BSDF sampling using one-sample MIS as described in Equ.\ref{eqn:target_mis} (Sec.\ref{sec:mis}).

\Comment{
\begin{figure}[!ht]
    \includegraphics[width=0.8\linewidth]{image/hash_grid.pdf}
    \caption{Path samples are traced to initialize empty maps and photon energy is splatted to those maps (a-b). The pre-trained neural network reconstructs high-quality density maps from the noisy energy maps (c), which are then used for guiding remaining path samples. To enable different caching granularity at different parts of the scene, we adaptively subdivide some voxels into smaller sub-voxels based on the collected photon statistics (d).}
    \label{fig:workflow}
\end{figure}
}

\begin{figure}[h]
    \includegraphics[width=\linewidth]{image/map_vis.pdf}
    \caption{The neural network architecture for density map reconstruction. We use a compact autoencoder which can extract high-level features from the input energy map and output a smooth and dense sampling map. The convolution uses circular padding on $\phi$ and replication padding on $z$. Each convolution (except for the last one) is followed by a batch normalization layer and a leaky ReLU activation layer.}
    \label{fig:net}
\end{figure}

\subsection{Spatial Caching}
\label{sec:cache}
In this section, we introduce our hash grid for storing the photon energy and density maps. We initially partition the scene into a fixed-resolution 3D hash grid that contains many equal-sized voxels. Each voxel covers a small volume of the scene and can be accessed by its index in the grid. This has two advantages: First, the hash grid can be built instantly with a reasonable initial resolution, which takes only a small amount of time; Second, the hash grid supports $O(1)$ access of each voxel, so it is fast to search the nearest density map in rendering. Note that we only allocate memory for voxels which contain actual scene surface and maps.

\paragraph{Photon energy deposit} We trace a batch of photons in each iteration and accumulate their energy into map $M_{e}$. Here, we use the cylindrical parameterization which converts the normalized photon direction $r=(x, y, z)$ to the floating-point 2D location ($p$, $q$) on $M_{e}$ as ($p$, $q$) $=$ ($z$, $\phi$) where $\phi=\arctan(y/x)$ since such transformation preserves area ratios. The photon energy is splatted and weighted by the distance to the 4 nearest bins on $M_{e}$ that surround ($p$, $q$) to deposit $s_{i}$ values based on Equ.\ref{eqn:store_weight_target} or Equ.\ref{eqn:store_weight_target_variance}. As mentioned in Equ.\ref{eqn:photon}, the accumulated photon energy of each bin on $M_{e}$ directly relates to the amount of incident energy that flows through the subtended solid angle $\Delta\omega$ and area $\Delta A$ that is shared by all the photons in the same voxel.

\paragraph{Cache update} The quality of the guided sampling direction is affected by the spatial resolution of stored density maps. Reusing the nearest density map brings error due to the location discrepancy. In other words, we need to ensure the reused density map is spatially close enough to the intersection point. In practice, different parts of the scene may require different caching granularity according to two factors: \textit{(i) number of photons: }if there are many photons in a voxel, this part of the scene probably has large contribution to pixel colors; \textit{(ii) variance of normals: }if the normal vectors of photons in a voxel have large variance, the local geometry probably has large curvature. In either case, we recursively subdivide the voxel into equal-sized 8 child voxels and each child can cache a new map. In this way, we allow higher caching granularity when necessary.

\paragraph{Density map reuse} To use the learned density maps for guiding path samples, we need to find the nearest one stored in the spatial cache for each intersection point. Thanks to our hash grid design, this is simple: reuse the density map stored in the voxel that contains the intersection point. If a child voxel does not contain any stored density map, we search along the subdivision hierarchy to use the density map stored in its parent voxel. According to our experiments, this is sufficient for generating good rendering results and keeping the path guiding running fast. Additionally, we can get better continuously-varying density maps in space by doing a distance-weighted linear interpolation of maps stored in multiple neighboring voxels. However, the weighted combination of multiple maps for each intersection point is computationally expensive on CPU renderers like Mitsuba, and we leave the fast implementation of such interpolation on GPU renderers like NVIDIA OPTIX \cite{parker2010optix} as future work (Sec.\ref{sec:discuss}).

\subsection{Target Density Reconstruction}
\label{sec:neural}
The raw energy map $M_{e}$ is usually noisy, which cannot represent the incident radiance well and could introduce artifacts in the rendering. Besides, we only have sparse photons in early iterations, so many bins in $M_{e}$ are empty. However, our target sampling density $M_{d}$ should be proportional to the continuous incident radiance as mentioned in Equ.~\ref{eqn:target} and Equ.~\ref{eqn:target_variance}. Therefore, we need to convert the noisy $M_{e}$ to a smooth and dense sampling map $M_{d}$. To solve this under-determined task, we choose to use neural network since it can learn from the past experience on the offline training data and predict the shape of the target density function based on the prior knowledge. 

\paragraph{Neural architecture} We have tried different neural network architectures, and we found Convolutional Neural Network (CNN) is the most robust choice for density map reconstruction. As illustrated in Fig.~\ref{fig:net}, we use a compact autoencoder~\cite{ronneberger2015u} architecture containing several convolutional layers to extract high-level features from the input energy map $M_{e}$ and output the reconstructed density map $M_{d}$. In addition, we record the number of photons and compute the average variance from groups of photon energy per bin on $M_{e}$, and use them as additional auxiliary features. Unlike previous screen-space methods, We empirically find that geometric features such as position, normal, and depth do not help too much here on our spatially-coherent local 3D voxels. Considering the limited caching memory and running time, we do not add more auxiliary features for now, and it is interesting for future research to explore more useful features on 3D voxels. After the density map is reconstructed, we compute PDF/CDF from it for importance sampling in guiding.

\paragraph{Dataset} To train our autoencoder, we procedurally generate 500 scenes with random objects, materials, and area lights. Each scene randomly picks one of 200 environment lights. Therefore, our training scenes contain the diverse geometry and light setups. To better adapt to the complex modern test scenes, we also collect 20 indoor and outdoor scenes used in previous works or obtained from modeling artists. Some example scenes are shown in Fig.\ref{fig:scenes}. For each scene, we construct multiple random-resolution hash grids. For each voxel, the ground-truth incident radiance is proportional to the incident photon energy as described in Equ.\ref{eqn:irradiance} since the area $\Delta A$ is constant for all the photons in the same voxel. Such incident energy is rendered by accumulating photons of 1M iterations, and the input maps are created by accumulating photons of random early iterations. To further augment the data, we randomly rotate the world coordinate frame. Moreover, values in both input maps and ground truth output maps are normalized to [0, 1] to stabilize the gradient descent optimization. The total number of training pairs in our dataset is about 10.5 million.
Note that we have two versions of stored $s_{i}$ values (Equ.\ref{eqn:store_weight_target} and Equ.\ref{eqn:store_weight_target_variance}) based on different target density functions (Equ.\ref{eqn:target} and Equ.\ref{eqn:target_variance}), and both input maps and ground-truth output maps are computed using the same formulation. For example, if variance-aware target density is used, then both input and output maps are converted to the square root of the second moment as described in Equ.\ref{eqn:store_weight_target_variance}. 

\paragraph{Loss function and training} We use the standard $l_{1}$ loss on the output density map:
\begin{equation}
    \mathbb{L} = \frac{1}{K}\sum_{i=1}^{K}|\hat{M_{d}} - M_{d}|
    \label{eqn:loss}
\end{equation}
where $K$ is the training batch size, $\hat{M_{d}}$ is the predicted density map, and $M_{d}$ is the ground-truth target density map. To avoid potential over-blurring, we also borrow the asymmetric loss function from previous denoising work \cite{vogels2018denoising}:
\begin{equation}
    \mathbb{L}_{\lambda} = \mathbb{L} \cdot (1 + (\lambda - 1) \cdot \mathbb{H})
    \label{eqn:loss_asym}
\end{equation}
where $\mathbb{H}=1$ if the output and the input are not on the same side relative to the ground truth and $\mathbb{H}=0$ otherwise. This function penalizes the output that diverges too much from the input. In our work, we empirically find $\lambda=1.5\sim2.5$ can yield reasonable output density maps with good sharpness.

In general, the photon distribution varies spatially in the scene. For example, there are many photons in the caustics area and very few photons in the shadow. Therefore, the input energy maps $M_{e}$ can have different levels of bias and variance at different locations. Since our autoencoder has limited capacity due to small size, it cannot perfectly handle the inputs with uneven qualities. To remediate this issue, we borrow the idea of the \textit{multiple local experts} \cite{jacobs1991adaptive} in machine learning where the entire system is composed of many separate 
networks/experts, each of which learns to handle a subset of the complete set of cases. Here, we train multiple versions of the same autoencoder (5 in our experiments), where the first one handles the most sparse photon inputs and the last one handles the most dense photon inputs. During the training and rendering, we split $M_{e}$ into multiple groups based on the number of accumulated photons of each map, and these networks reconstruct density maps in parallel on multiple GPUs.

\subsection{Multiple Importance Sampling}
\label{sec:mis}
Similarly to previous path guiding work, the reconstructed densities only consider the incident radiance, so we also need to combine it with BSDF sampling using one-sample MIS (Equ.\ref{eqn:target_mis}):
\begin{equation}
    \begin{split}
    p(\DirI) & = \alpha p_{\text{BSDF}}(\DirI) + (1-\alpha)p_{\text{guide}}(\DirI) \\
                    & = \frac{\nu_{\text{BSDF}}}{\nu_{\text{BSDF}} + \nu_{\text{Guide}}} p_{\text{BSDF}}(\DirI) + \frac{\nu_{\text{Guide}}}{\nu_{\text{BSDF}} + \nu_{\text{Guide}}}p_{\text{guide}}(\DirI)
    \end{split}
    \label{eqn:mis_coef}
\end{equation}
where $\nu_{\text{BSDF}}$ and $\nu_{\text{Guide}}$ represent the average product of BSDF value and incident radiance (i.e., $L_{i}(\Px, \DirI)\cdot f_{r}(\Px, \DirI, \DirO)$) over the previous BSDF and guiding sampled path rays respectively. In the beginning, we always start with $p(\DirI) = 0.5\cdot p_{\text{BSDF}} + 0.5\cdot p_{\text{guide}}$ where guiding and BSDF have equal chances to be selected for importance sampling. When enough reflected rays have been sampled, we update the mixture coefficient $\alpha$ based on Equ.~\ref{eqn:mis_coef}. Furthermore, we clamp $\alpha$ to $[0.2, 0.8]$, and we only use BSDF sampling if the surface is a mirror or glass.


}



































==> 3-method.tex <==
\section{Background}
\label{sec:background}
In this section, we review the important concepts of Monte Carlo integration and importance sampling, and discuss the target density function in path guiding. We also describe the concept of photons since they are the primary source of input in our proposed system.

Physically-based rendering can be expressed by the Rendering Equation \cite{kajiya1986rendering} at each intersection point $\bm x$:
\begin{equation}
    L(\bm x, \omega_{o}) = L_{e}(\bm x, \omega_{o}) + \int_{\Omega}L_{i}(\bm x, \omega_{i})f_{r}(\bm x, \omega_{i}, \omega_{o})|\cos\theta_{i}|d\omega_{i},
    \label{eqn:re}
\end{equation}
where $L_{e}(\bm x, \omega_{o})$ denotes the emitted radiance from point $\bm x$ in direction $\omega_{o}$, and $f_{r}$ is the bidirectional scattering distribution function (BSDF). This equation describes the relation between the outgoing radiance $L(\bm x, \omega_{o})$ and the incident radiance $L_{i}(\bm x, \omega_{i})$ over the hemisphere $\Omega$. By importance sampling the incident direction $\omega_{i}$, the outgoing radiance $L(\bm x, \omega_{o})$ can be approximated as \cite{veach1997robust}:
\begin{equation}
    L_{r}(\bm x, \omega_{o}) = \frac{1}{N} \sum_{i=1}^{N} \frac{L_{i}(\bm x, \omega_{i})f_{r}(\bm x, \omega_{i}, \omega_{o})|\cos\theta_{i}|}{p(\omega_{i})}
    \label{eqn:mc}
\end{equation}
where $L_{r}(\bm x, \omega_{o})$ is the estimated outgoing radiance, $N$ is the total number of Monte Carlo samples, and $p(\omega_{i})$ is the probability density function (PDF) of sampling $\omega_{i}$. In Monte Carlo path tracing, we sample a reflected or refracted ray from each intersection point and use Equ.\ref{eqn:mc} to compute the radiance that contributes to the pixel color. 

The variance of the Monte Carlo estimated radiance $L_{r}(\bm x, \omega_{o})$ can be reduced by sampling $\omega_{i}$ from a density function $p(\omega_{i})$ that resembles the numerator $L_{i}(\bm x, \omega_{i})f_{r}(\bm x, \omega_{i}, \omega_{o})|\cos\theta_{i}|$. Ideally, if $p(\omega_{i})$ and the numerator only differs by a constant scale, the variance is reduced to zero. Therefore, path guiding aims to reconstruct a density function that matches the shape of this numerator as close as possible. Additionally, since BSDF importance sampling satisfies $p_{\text{BSDF}}(\omega_{i}) \propto f_{r}(\bm x, \omega_{i}, \omega_{o})$, previous path guiding methods often set the target density to be proportional to the incident radiance \cite{muller2017practical, vorba2014line, bako2019offline}:
\begin{equation}
    p_{\text{guide}}(\omega_{i}) \propto L_{i}(\bm x,   \omega_{i})|\cos\theta_{i}|
    \label{eqn:target}
\end{equation}
and then combine guided sampling with BSDF sampling using the one-sample Multiple Importance Sampling (MIS) \cite{veach1995optimally}:
\begin{equation}
    p(\omega_{i}) = \alpha p_{\text{BSDF}}(\omega_{i}) + (1-\alpha)p_{\text{guide}}(\omega_{i})
    \label{eqn:target_mis}
\end{equation}
where $\alpha$ is the mixture coefficient that determines the probability of choosing BSDF over guiding for importance sampling. In practice, path guiding uses early path samples to compute a good estimation of $L_{i}(\bm x, \omega_{i})$, and remaining samples are guided by importance sampling using Equ.\ref{eqn:target_mis}.
Very recently, \citet{Rath2020} observes that it is often infeasible to perfectly obtain the target density (Equ.\ref{eqn:target}) for every intersection point in practice. Thus, the variance of $L_{i}(\bm x, \omega_{i})$ should also be considered, which leads to the square root of the second moment:
\begin{equation}
    p_{\text{guide-variance-aware}}(\omega_{i}) \propto \sqrt{\mathbb{E}[L_{i}^{2}(\bm x, \omega_{i})]}|\cos\theta_{i}|
    \label{eqn:target_variance}
\end{equation}
In fact, the choice between Equ.\ref{eqn:target} and Equ.\ref{eqn:target_variance} is orthogonal to our proposed framework. In this paper, we develop two versions of our system where the \textit{radiance version} uses Equ.\ref{eqn:target} and the \textit{variance version} uses Equ.\ref{eqn:target_variance} as the target density function. Integrating more advanced functions such as the \textit{full target density} proposed in \citet{Rath2020} into our system is left for future work.

In practice, however, we can only store a discrete set of $s_{i}$ where each one represents the total amount of incident radiance with respect to a finite subtended solid angle $\Delta\omega$:
\begin{equation}
    E_{i}(\bm x, \Delta\omega) = \int_{\Delta\omega} L_{i}(\bm x, \omega_{i})|\cos\theta_{i}|d\omega_{i}
    \label{eqn:irradiance} = \frac{\Phi}{\Delta A}
\end{equation}
this is the \textit{irradiance} $E_{i}$ which indicates the amount of incident \textit{energy} $\Phi$ per unit area that flows through $\Delta\omega$. Therefore, for target density Equ.\ref{eqn:target} and Equ.\ref{eqn:target_variance}, the stored value $s_{i}$ can be written as:
\begin{equation}
    s_{i} \propto \int_{\Delta\omega} p_{\text{guide}}(\omega_{i})d\omega_{i}
    \label{eqn:store_weight_target}
\end{equation}
and
\begin{equation}
    s_{i} \propto \sqrt{|\Delta\omega|\int_{\Delta\omega} p_{\text{guide-variance-aware}}^{2}(\omega_{i})d\omega_{i}}
    \label{eqn:store_weight_target_variance}
\end{equation}

In some challenging light transport scenarios, it can be hard to get a good estimated $L_{i}(\bm x, \omega_{i})$ from a small number of path samples, thus learning the target density will become slow (i.e., cold start problem). In these cases, using photons is often a better choice. Photons are particles emitted from light sources. Each photon carries a partial energy (i.e., flux) $\Delta\Phi$ of the light's power and a direction that roughly indicates where the radiance comes from \cite{jensen1995importance}. After photons leave the light source, they are bounced and distributed within the scene. When a photon hits a diffuse or glossy surface, it is stored at the intersection point on the surface. In general, the stored photons can approximately represent the incident radiance distribution at each intersection point $\bm x$:
\begin{equation}
    L_{i}(\bm x, \omega_{i} | \omega_{i} \in \Delta\omega) \approx \frac{1}{\Delta\omega \Delta A \cos\theta_{i}}\sum_{p=1}^{m}\Delta\Phi_{p} \propto \frac{1}{\Delta\omega \cos\theta_{i}}\sum_{p=1}^{m}\Delta\Phi_{p}
    \label{eqn:photon}
\end{equation}
where $m$ is the number of photons that come from a set of directions $\Delta\omega$ and stored in the neighboring region $\Delta A$ of $\bm x$, and $\Delta\Phi_{p}$ is the energy flux carried by the photon $p$. In this work, we use photon energy to estimate $L_{i}(\bm x, \omega_{i})$ and reconstruct the target density function (Equ.\ref{eqn:target} and Equ.\ref{eqn:target_variance}) by storing discrete $s_{i}$ values (Equ.\ref{eqn:store_weight_target} and Equ.\ref{eqn:store_weight_target_variance}) in a spatial cache. Based on our experiments (Sec.\ref{sec:eval}), our photon-driven system works well for challenging scenes with complex lightings, especially where path samples are difficult to find the light sources while photons are easily reachable. Besides, photon-driven methods can better explore the entire sampling space, while path sample based methods may get stuck in a sampling direction once a light source is found which is similar to the local exploration issue in Metropolis light transport.  

\section{Method}
\label{sec:method}

\subsection{System Overview}
\begin{figure}[!ht]
    \includegraphics[width=\linewidth]{image/system.pdf}
    \caption{We train our system iteratively to learn sampling density maps and store them in a spatial cache. In every iteration, path samples are generated from the camera, and photons are emitted from light sources. Path samples determine where to create new energy map in the scene, and energy of each photon is deposited to the nearest map in the spatial cache. These energy maps then pass through a pre-trained neural network that can reconstruct dense sampling maps which are then used for guiding remaining path samples in training and rendering. Furthermore, the spatial cache that stores the maps is updated on-the-fly through iterations.}
    \label{fig:system}
\end{figure}

The entire proposed system is summarized in Fig. \ref{fig:system}. We first learn target sampling densities $p(\omega_{i})$ at different locations in the scene through iterative training. After the training is completed, we use the learned densities to guide path samples in both the remaining training and rendering. At the beginning, the scene is partitioned into many small voxels using a fixed-resolution 3D hash grid. These voxels are used for caching the learned densities at different locations (Sec.\ref{sec:cache}). Here, we use 2D images to store $s_{i}$
and density values, where each bin/pixel ($i$, $j$) represents a subset of incident directions $\{ \omega_{i} | \omega_{i} \in \Delta\omega \}$ over a sphere. We will call these stored images as \textit{maps} in the rest of this paper.

During training, we trace path samples and adaptively initialize the maps. For every intersection point, if a map does not exist in the voxel that contains the point, an empty map $M_{e}$ is created and cached in the voxel. Next, photons are emitted from the light sources. Since photons can represent the incident radiance field (Equ.\ref{eqn:photon}), we reconstruct $L_{i}(\bm x, \omega_{i})$ from neighboring photons at each intersection point $\bm x$ by mapping each photon's direction to a 2D position on $M_{e}$ and splatting its energy $\Delta\Phi$ to $M_{e}$ (Sec.\ref{sec:cache}). In other words, every bin on $M_{e}$ stores the $s_{i}$ value in Equ.\ref{eqn:store_weight_target} or Equ.\ref{eqn:store_weight_target_variance} representing the incident energy that flows through the bin. After the energy is consumed by the map, the photon is deleted from the memory.

We observe that $M_{e}$ is usually quite noisy since photons are discrete samples of light power. Therefore, we train a neural network that takes these noisy maps as inputs and reconstructs the dense and smooth sampling maps $M_{d}$ (Sec.\ref{sec:neural}). The network is trained on offline data using either Equ.\ref{eqn:target} or Equ.\ref{eqn:target_variance} as the ground-truth output. This neural network reconstruction is only executed to update $M_{d}$ when enough amount of new photon energy is consumed into $M_{e}$ after every several new iterations. Since $M_{e}$ gets continuously improved over iterations by consuming more photons, the latest reconstructed $M_{d}$ also gets better over time. After reconstruction, $M_{d}$ are stored in the voxels and used to guide remaining path samples by allowing intersection points to reuse the cached density maps $M_{d}$ for importance sampling. 

Thanks to our spatial hash grid, each voxel can be accessed by its index in $O(1)$ time. Therefore, depositing photon energy and searching nearest density map $M_{d}$ are faster on our hash grid than on tree structures. Furthermore, we adaptively subdivide the voxels into smaller ones based on the collected photon statistics to allow different caching granularity at different parts of the scene, which can be seen as the combination of the hash grid and the hierarchical tree (Sec.\ref{sec:cache}). 

After training is completed, the learned density maps $M_{d}$ are used to guide path samples in rendering. For each intersection point, the reflected ray is importance sampled from the nearest cached $M_{d}$. Since the reconstructed density maps can contain zeros, we combine the guiding sampling with BSDF sampling using one-sample MIS as described in Equ.\ref{eqn:target_mis} (Sec.\ref{sec:mis}).

\Comment{
\begin{figure}[!ht]
    \includegraphics[width=0.8\linewidth]{image/hash_grid.pdf}
    \caption{Path samples are traced to initialize empty maps and photon energy is splatted to those maps (a-b). The pre-trained neural network reconstructs high-quality density maps from the noisy energy maps (c), which are then used for guiding remaining path samples. To enable different caching granularity at different parts of the scene, we adaptively subdivide some voxels into smaller sub-voxels based on the collected photon statistics (d).}
    \label{fig:workflow}
\end{figure}
}

\begin{figure*}[t]
    \includegraphics[width=\linewidth]{image/map_vis.pdf}
    \caption{The neural network architecture for density map reconstruction. We use a compact autoencoder which can extract high-level features from the input energy map and output a smooth and dense sampling map. The convolution uses circular padding on $\phi$ and replication padding on $z$. Each convolution (except for the last one) is followed by a batch normalization layer and a leaky ReLU activation layer.}
    \label{fig:net}
\end{figure*}

\subsection{Spatial Caching}
\label{sec:cache}
In this section, we introduce our hash grid for storing the photon energy and density maps. We initially partition the scene into a fixed-resolution 3D hash grid that contains many equal-sized voxels. Each voxel covers a small volume of the scene and can be accessed by its index in the grid. This has two advantages: First, the hash grid can be built instantly with a reasonable initial resolution, which takes only a small amount of time; Second, the hash grid supports $O(1)$ access of each voxel, so it is fast to search the nearest density map in rendering. Note that we only allocate memory for voxels which contain actual scene surface and maps.

\paragraph{Photon energy deposit} We trace a batch of photons in each iteration and accumulate their energy into map $M_{e}$. Here, we use the cylindrical parameterization which converts the normalized photon direction $r=(x, y, z)$ to the floating-point 2D location ($p$, $q$) on $M_{e}$ as ($p$, $q$) $=$ ($z$, $\phi$) where $\phi=\arctan(y/x)$ since such transformation preserves area ratios. The photon energy is splatted and weighted by the distance to the 4 nearest bins on $M_{e}$ that surround ($p$, $q$) to deposit $s_{i}$ values based on the radiance-based target density Equ.\ref{eqn:store_weight_target}. If the variance-based target density Equ.\ref{eqn:store_weight_target_variance} is used, then we uniformly splat the photon energy into neighboring pixels without weighing since the estimated variance can be negatively affected by the assigned weights. As mentioned in Equ.\ref{eqn:photon}, the accumulated photon energy of each bin on $M_{e}$ directly relates to the amount of incident energy that flows through the subtended solid angle $\Delta\omega$ and area $\Delta A$ that is shared by all the photons in the same voxel.

\paragraph{Cache update} The quality of the guided sampling direction is affected by the spatial resolution of stored density maps. Reusing the nearest density map brings error due to the location discrepancy. In other words, we need to ensure the reused density map is spatially close enough to the intersection point. In practice, different parts of the scene may require different caching granularity according to two factors: \textit{(i) number of photons: }if there are many photons in a voxel, this part of the scene probably has large contribution to pixel colors; \textit{(ii) variance of normals: }if the normal vectors of photons in a voxel have large variance, the local geometry probably has large curvature. In either case, we recursively subdivide the voxel into equal-sized 8 child voxels and each child can cache a new map. In contrast to the hierarchical subdivision, when a voxel has too few photons (e.g., less than 10), the photons of its one-surrounding nearest voxels are also collected to reduce sparsity and a new parent voxel is created for it. This adaptive subdivision and merging allows different caching granularity when necessary. Note that subsequent photon energy is deposited into both parent and child voxels if a hierarchy exists at the photon's location.

\paragraph{Density map reuse} To use the learned density maps for guiding path samples, we need to find the nearest one stored in the spatial cache for each intersection point. Thanks to our hash grid design, this is simple: reuse the density map stored in the voxel that contains the intersection point. If a child voxel does not contain any stored density map or enough amount of accumulated photons, we search along the subdivision hierarchy to use the density map stored in its parent voxel. According to our experiments, this is sufficient for generating good rendering results and keeping the path guiding running fast. After obtaining the nearest density map, we use the linearly interpolated importance sampling to draw a new direction. Additionally, we can get better continuously-varying density maps in space by doing a distance-weighted linear interpolation of maps stored in multiple neighboring voxels. However, the weighted combination of multiple maps for each intersection point is computationally expensive on CPU renderers like Mitsuba, and we leave the fast implementation of such interpolation on GPU renderers like NVIDIA OPTIX as future work (Sec.\ref{sec:discuss}).

\subsection{Target Density Reconstruction}
\label{sec:neural}
The raw energy map $M_{e}$ is usually noisy, which cannot represent the incident radiance well and could introduce artifacts in the rendering. Besides, we only have sparse photons in early iterations, so many bins in $M_{e}$ are empty. However, our target sampling density $M_{d}$ should be proportional to the continuous incident radiance as mentioned in Equ.~\ref{eqn:target} and Equ.~\ref{eqn:target_variance}. Therefore, we need to convert the noisy $M_{e}$ to a smooth and dense sampling map $M_{d}$. To solve this under-determined task, we choose to use neural network since it can learn from the past experience on the offline training data and predict the shape of the target density function based on the prior knowledge. 

\paragraph{Neural architecture} We have tried different neural network architectures, and we found Convolutional Neural Network (CNN) is the most robust choice for density map reconstruction. As illustrated in Fig.~\ref{fig:net}, we use a compact autoencoder~\cite{ronneberger2015u} architecture containing several convolutional layers to extract high-level features from the input energy map $M_{e}$ and output the reconstructed density map $M_{d}$. In addition, we record the fractional number of photons (i.e., summed distance-based weights to 4 nearest pixels during energy splatting) and the variance of photon energy per bin on $M_{e}$, and use them as additional auxiliary features. These features generally help to disambiguate the incident energy and perform different levels of denoising on different parts of the map. Furthermore, unlike screen-space methods, we find that geometric features such as the average depth and shading normal from the previous photon bounce offer slight improvement on simple scenes but large increment in memory usage, and for many of our complex test scenes some of these signals can be noisy and incoherent due to the high geometric variation rate compared to the voxel size. Therefore, we temporarily exclude these geometric features, and it is interesting for future research to explore more useful features on 3D voxels. After the density map is reconstructed, we compute PDF/CDF from it for importance sampling in guiding.

\paragraph{Dataset} To train our autoencoder, we procedurally generate 500 scenes with random objects, materials, and area lights. Each scene randomly picks one of 200 environment lights. Therefore, our training scenes contain the diverse geometry and light setups. To better adapt to the complex modern test scenes, we also collect 20 indoor and outdoor scenes used in previous works or obtained from modeling artists. Some example scenes are shown in Fig.\ref{fig:scenes}. For each scene, we construct multiple random-resolution hash grids. For each voxel, the ground-truth incident radiance is proportional to the incident photon energy as described in Equ.\ref{eqn:irradiance} since the area $\Delta A$ is constant for all the photons in the same voxel. Such incident energy is rendered by accumulating photons of 1M iterations, and the input maps are created by accumulating photons of random early iterations. To further augment the data, we randomly rotate the world coordinate frame. Moreover, values in both input maps and ground truth output maps are normalized to [0, 1] to stabilize the gradient descent optimization. The total number of training pairs in our dataset is about 10.5 million.
Note that we have two versions of stored $s_{i}$ values (Equ.\ref{eqn:store_weight_target} and Equ.\ref{eqn:store_weight_target_variance}) based on different target density functions (Equ.\ref{eqn:target} and Equ.\ref{eqn:target_variance}), and both input maps and ground-truth output maps are computed using the same formulation. For example, if variance-aware target density is used, then both input and output maps are converted to the square root of the second moment as described in Equ.\ref{eqn:store_weight_target_variance}. 

\paragraph{Loss function and training} We use the standard $l_{1}$ loss on the output density map:
\begin{equation}
    \mathbb{L} = \frac{1}{K}\sum_{i=1}^{K}|\hat{M_{d}} - M_{d}|
    \label{eqn:loss}
\end{equation}
where $K$ is the training batch size, $\hat{M_{d}}$ is the predicted density map, and $M_{d}$ is the ground-truth target density map. To avoid potential over-blurring, we also borrow the asymmetric loss function from previous denoising work \cite{vogels2018denoising}:
\begin{equation}
    \mathbb{L}_{\lambda} = \mathbb{L} \cdot (1 + (\lambda - 1) \cdot \mathbb{H})
    \label{eqn:loss_asym}
\end{equation}
where $\mathbb{H}=1$ if the output and the input are not on the same side relative to the ground truth and $\mathbb{H}=0$ otherwise. This function penalizes the output that diverges too much from the input. In our work, we empirically find $\lambda=1.5\sim2.5$ can yield reasonable output density maps with good sharpness.

In general, the photon distribution varies spatially in the scene. For example, there are many photons in the caustics area and very few photons in the shadow. Therefore, the input energy maps $M_{e}$ can have different levels of bias and variance at different locations. Since our autoencoder has limited capacity due to small size, it cannot perfectly handle the inputs with uneven qualities. To remediate this issue, we borrow the idea of the \textit{multiple local experts} \cite{jacobs1991adaptive} in machine learning where the entire system is composed of many separate 
networks/experts, each of which learns to handle a subset of the complete set of cases. Here, we train multiple versions of the same autoencoder (4 in our experiments), where the first one handles the most sparse photon inputs and the last one handles the most dense photon inputs. During the training and rendering, we split $M_{e}$ into multiple groups based on the number of accumulated photons of each map, and these networks reconstruct density maps in parallel on multiple GPUs.

\subsection{Multiple Importance Sampling}
\label{sec:mis}
Similarly to previous path guiding work, the reconstructed densities only consider the incident radiance, so we also need to combine it with BSDF sampling using one-sample MIS (Equ.\ref{eqn:target_mis}):
\begin{equation}
    \begin{split}
    p(\omega_{i}) & = \alpha p_{\text{BSDF}}(\omega_{i}) + (1-\alpha)p_{\text{guide}}(\omega_{i}) \\
                    & = \frac{\nu_{\text{BSDF}}}{\nu_{\text{BSDF}} + \nu_{\text{Guide}}} p_{\text{BSDF}}(\omega_{i}) + \frac{\nu_{\text{Guide}}}{\nu_{\text{BSDF}} + \nu_{\text{Guide}}}p_{\text{guide}}(\omega_{i})
    \end{split}
    \label{eqn:mis_coef}
\end{equation}
where $\nu_{\text{BSDF}}$ and $\nu_{\text{Guide}}$ represent the average product of BSDF value and incident radiance (i.e., $L_{i}(\bm x, \omega_{i})\cdot f_{r}(\bm x, \omega_{i}, \omega_{o})$) over the previous BSDF and guiding sampled path rays respectively. In the beginning, we always start with $p(\omega_{i}) = 0.5\cdot p_{\text{BSDF}} + 0.5\cdot p_{\text{guide}}$ where guiding and BSDF have equal chances to be selected for importance sampling. When enough reflected rays have been sampled, we update the mixture coefficient $\alpha$ based on Equ.~\ref{eqn:mis_coef}. Furthermore, we clamp $\alpha$ to $[0.2, 0.8]$, and we only use BSDF sampling if the surface is a mirror or glass.






































==> 4-eval.tex <==
\section{Evaluation}
\label{sec:eval}

Now, we show the performance of our proposed system on 12 representative test scenes. Here, we show visual comparisons on some exemplary image patches for each scene and additional results can be found in the supplementary document. All scenes are modified to contain various challenging lights that are difficult for the standard path tracing to search. In this work, we compare results rendered with medium to high sample count, since very noisy low sample count results are less useful in practice such as film productions. Unless otherwise stated, Next event estimation (NEE) is disabled in default since most parts of the scene have poor visibility to light sources, which was also the default choice in previous work \cite{vorba2014line, muller2017practical} to emphasize the difference in guiding distributions. For indoor room scenes lit by an outdoor environment sunlight, photons are emitted by importance sampling directions towards the windows, unless otherwise stated in the guided photon tracing extension. The effects of these modules are studied in the supplementary document.


\paragraph{Quantitative comparisons. }
Table \ref{tab:quant_rmse} presents the quantitative results on all of our tested scenes. For each scene, we compute the rMSE and SSIM over the full-resolution rendered image. As shown from the results, our proposed system performs the best. Since most of our test scenes have strong indirect radiance contribution to the pixel colors, first-bounce guiding like \cite{bako2019offline} is not very effective. For some scenes like \textsc{Spaceship} and \textsc{Living room} where many small lights are hidden behind glass objects, it is a lot more beneficial to use photons instead of path samples to learn sampling maps by \cite{vorba2014line} and our method. For general scenes, \cite{muller2017practical} is often better than \cite{vorba2014line} due to the much better SD-Tree caching structure. By considering the variance of the incident radiance, \cite{Rath2020} usually outperforms \cite{muller2017practical} due to the more advanced variance-aware target density function. Next, we use some representative cropped regions for visual comparisons.

\paragraph{Transparent objects. }
In many challenging light transport cases which involve transmission and reflection of transparent objects, photon-driven methods can be very effective. As shown in Fig.\ref{fig:transparent}, the \textsc{Spaceship} scene contains glass windshields and multiple glowing components. The \textsc{Caustics Egg} scene produces strong caustics on the diffuse table caused by the glass egg. The \textsc{Wild Creek} scene also contains strong caustics under both the water and diamond rocks. These challenging light transport cases make path samples very difficult to find the lights, but neighboring photons are easily reachable. Therefore, both our proposed method and \cite{vorba2014line} produce good results in those caustics regions. First-bounce guiding method like \cite{bako2019offline} does not significantly improve the results since many pixel colors are contributed by the indirect bounces in these scenes. Although \cite{muller2017practical} and \cite{Rath2020} can reduce the pixel noise effectively due to the use of better SD-Tree caching structure and advanced variance aware target density, they still suffer from the limitation of path samples and higher levels of noise in the sampling map compared with the smooth neural network reconstruction. 

\paragraph{Complex lighting. }
Real scenes can contain complex light sources, and some of them are shown in Fig.\ref{fig:complex_light}. The \textsc{Bathroom} scene has four spherical area lights in the glass bulbs and one sunlight outside the irregularly-occluded window. The \textsc{Kitchen} scene is illuminated by a sunlight through a window, and seven small area lights that illuminate the kitchen countertop. The \textsc{Staircase} scene is lit by two area lights from the backside room and downstairs respectively, as well as eight decorative lights on the ceiling and walls. In all of these scenes, the incident radiance comes from multiple directions and is often very noisy, so learning and rendering can take more time since contributions from multiple lights must be added together. Here, path sample based methods like \cite{muller2017practical}, \cite{bako2019offline} and \cite{Rath2020} are also effective. Since \cite{vorba2014line} uses Gaussian Mixture Model (GMM) that naturally has lower resolution in early iterations, the reconstructed sampling maps can be less accurate when the incident radiance becomes complex. Their rendering speed is also slower than \cite{muller2017practical}'s SD-tree and our voxelized grid due to the heavy usage of nearest neighbor search in a giant tree. As we already stated, \cite{bako2019offline} can effectively improve the first bounce sampling quality but fail to handle indirect bounces, leading to worse performance compared to other baselines. As for \cite{muller2017practical} and \cite{Rath2020}, the major drawback is to build the SD-tree from scratch which consumes more time than our method during online learning. In contrast, our system can reconstruct better sampling maps with enough resolution for arbitrary bounces and efficiently store them in spatially-coherent 3D voxels for importance sampling. Therefore, we can achieve better results with the same amount of time even under such complex lighting scenarios.

\paragraph{Equal quality comparison. }
In addition to the equal-time comparison, we also compare the time spent to achieve results of similar quality on some most notoriously challenging scenes we have. For such equal-quality comparison, we mainly focus on comparing to the baseline methods that support guiding arbitrary bounces, since the path tracing and first-bounce guiding methods like \cite{bako2019offline} can take substantial amount of time when the pixel color is dominated by contribution of the indirect bounces. As shown in Fig.\ref{fig:budget}, the \textsc{Veach Ajar} scene is very tough to render since there is only one light source illuminating the entire scene through a small slit. The \textsc{Living Room} scene has multiple lights on the flower and inside the glass bottles on the wall cabinet. The \textsc{Hotel} scene has multiple ceiling lights and 2 lamp lights where most of them are completely concealed by at least one layer of casing. In all of these cases, we continuously run more training iterations for \cite{vorba2014line}, \cite{muller2017practical} and \cite{Rath2020} until the produced whole image is comparable to the one generated by our best system (rMSE difference < $10^{-4}$). 

\paragraph{Temporal stability. }
We also compare the temporal stability with respect to the camera movement. The performance on animated scenes is left for future work.
As shown in Fig.\ref{fig:temporal}, the \textsc{Torus} scene has a diffuse object wrapped in a glass cube and produces caustics underneath. The inside torus is hard to render for path tracing due to Specular-Diffuse-Specular (SDS) paths. Following the previous denoising work \cite{vogels2018denoising}, we use the mean DSSIM (i.e., dissimilarity) between consecutive frames to evaluate the temporal consistency when fast moving the camera. From the results we can see lower variance results often lead to better temporal consistency. Future research can extend our system by adding recurrent neural architectures to explicitly relate neighboring frames.

\begin{figure}[h]
    \includegraphics[width=\linewidth]{image/temporal.pdf}
    \caption{Average DSSIM (lower is better) computed from 30 consecutive frames when the camera is moving fast along a direction. The dissimilarity is affected by both the content change as well as the noise level.}
    \label{fig:temporal}
\end{figure}

\begin{figure*}[t]
    \includegraphics[width=\linewidth]{image/ablation.pdf}
    \caption{We study the effectiveness of the neural reconstruction module. Without neural sampling map reconstruction, the results have higher noise level. Moreover, the resolution of the sampling map also slightly affects the performance.}
    \label{fig:ablation}
\end{figure*}

\paragraph{Sampling map reconstruction}
Next, we study the effect of the proposed neural reconstruction framework. As shown in Fig.\ref{fig:ablation}, the \textsc{Pool} scene has glossy floor and detailed caustics under the water, which is lit by an environment sunlight. The \textsc{Classroom} scene has the same outdoor sunlight and a ceiling projector that emits blue lights. To study the effectiveness of the neural reconstruction module, we temporarily remove it from the system, and use the raw deposited maps directly for importance sampling to compare against the neural reconstructed density maps. In addition, we reconstruct sampling maps with different resolutions, $32\times64$ and $64\times128$ respectively, to study the effect of solid angle granularity to the final rendering results. 

\paragraph{Spatial grid partitioning}
\begin{figure}[h]
    \includegraphics[width=\linewidth]{image/partition_grid.pdf}
    \caption{The effect of initial grid resolution and our hierarchical spatial partitioning framework. Ideally, the voxel size should be small enough to reflect the locality of the incident radiance, and large enough to contain enough photons for sampling map reconstruction. In the extreme case, under-partitioning and over-partitioning will both hurt the performance.}
    \label{fig:grid}
\end{figure}

Finally, we investigate the proposed spatial caching structure - the hierarchical grid. Unlike previous methods which start from a giant bounding box that covers the entire scene and gradually refine the spatial SD-Tree \cite{muller2017practical, Rath2020}, our hash grid has fixed resolution in the beginning so that our method takes less time and iterations to finish the construction of a good spatial cache. Moreover, our spatial partitioning mechanism allows each voxel to further adapt to the local geometry and lighting. We try different initial grid resolutions with or without partitioning and see how the setting affects rendering result. We believe this brings an interesting question on how to quickly partition the space into effective regions in the very beginning where each region has enough photons for sampling map reconstruction. 

\paragraph{Runtime distribution}
\begin{table}[h]
	\begin{center}
		%\resizebox{\linewidth}{!}{
		
		\begin{tabular}{p{0.3in}|p{0.6in}P{0.5in}P{0.5in}|P{0.7in} }  
			%\multicolumn{10}{|c|}{\Scenea}\\
			\hline  %\STAB{\rotatebox[origin=c]{90}{\Scenea}}
			& Path tracing (learning) & Photon tracing  & Neural rec & Path tracing (final-pass) \\
			\hline
			%\cline{2-10}
			Range & & &   & \\
			\hline
			Avg & & &   & \\
			\hline
		\end{tabular}
		%}
		\caption{Runtime distribution of different parts in the proposed system.}
		\label{tab:runtime}
	\end{center}
\end{table}

Thanks to our optimized CPU and GPU implementation that collaborates and parallelizes computations in rendering and neural network inference, the whole system can take the full load of these computing power. Since the absolute rendering time differs among scenes with different complexities, we concentrate on the relative portion of running time of each part in our system. The timing distribution in Table.~\ref{tab:runtime} is measured on a cluster with Intel Core i9-7960X CPU (2.80GHz), Nvidia Titan RTX GPUs (24GB), and 128GB system memory. 

In the supplementary material, we also study the effect of Monte-Carlo denoising, Next Event Estimation (NEE), neural architecture, one-sample MIS, and guided photon tracing extension. In addition, we present extra sampling map visualizations and discuss potential future extensions of our proposed system. Please refer to the supplementary document for detailed evaluations and discussion.




==> 5-app.tex <==
\section{Limitations, Conclusion and Future Work}
\label{sec:discuss}
In this paper, we presented a new full-bounce path guiding system that uses neural networks to reconstruct sampling density maps stored in an adaptive hash grid. Our system achieves promising performance in practice, and opens many appealing directions for future research. 
%In this section, we discuss some limitations of our system and possible ways to resolve them in the future.

\paragraph{System overhead. }
In this work, we use hash grid to cache the learned densities. Although the hash grid supports fast access through indexing, it can over-partition the scene and hence use more memory than baseline methods (consumes dozens of GBs in our experiments). We think this is a trade-off between the memory usage and the learning speed. If we start with a very coarse grid, then it will take more time to refine the voxels and the hierarchy will be much deeper so that locating a voxel will take more time, although the memory usage is reduced. Future research should search for the most balanced way to construct an optimal spatial cache based on the geometry and light setups. We also find that running network and the data transfer between CPU and GPU still take some time even on GPUs. Therefore, our current system on Mitsuba works well for medium to high sample counts when majority of timing is spent for tracing rays, but is not very effective for very low sample counts when the neural reconstruction becomes the timing bottleneck. Immigrating our system to a pure GPU renderer like Nvidia OPTIX is a straightforward solution. Future research can focus on designing useful metrics to decide how many iterative reconstructions are needed for different parts of the scene and when to stop the training automatically without user's guidance, which may effectively reduce the unnecessary network inference and save more sample counts for rendering. 

\paragraph{Bidirectional sample deposit. }
Since our current system is solely photon-driven, sometimes it can be affected by the limitation of photons. In some special cases where most photons are invisible to the camera, we have to add an extra guided photon tracing module to relieve the sparsity problem (Sec.\ref{sec:eval}). Such limitation may also exist when we only render a small part of a large-scale scene since many photons may never be used. In these special cases, path samples can be more efficient since they originate from the camera. Therefore, it is necessary to deposit both path samples and photons into an unified map followed by the neural density reconstruction, so that the whole system can work well for scenes with arbitrary geometry and lighting setup. A straightforward way is to combine our photon-driven neural path guiding with path sample based neural path guiding proposed by \cite{bako2019offline} (after extending their work to support multi-bounce guiding). Future research can also focus on learning to cleverly split the rendering budget into path samples and photons based on the properties of each individual scene.

\paragraph{Target density reconstruction. }
In some cases, a better target density function is more important. Due to the orthogonality, our method can be improved by more advanced density functions such as the \textit{full target density} proposed in \cite{Rath2020}. The screen-space adaptive sampling techniques (\cite{huo2020adaptive}) may also be integrated into our system for the first bounce to further reduce the variance of each pixel. Another direction to improve our system is to train a novel recurrent neural network which takes both the previous reconstructed map and new photon energy as inputs. In this way, we can reduce the memory usage by only keeping a single map per voxel. Another topic worth exploring is hierarchical density map reconstruction. In this work, our stored maps have a fixed resolution of 64 by 128, since we use the standard CNN that can only output a regular grid image. However, this is not ideal because the grid image contains redundant values. As proposed by \cite{muller2017practical}, it is desirable to have an adaptive directional density map where brighter bins get subdivided into smaller ones and darker bins remain big. Developing a novel neural network that can predict a hierarchical density map or a compressed representation of a density map instead of a regular grid image has not been explored and is worth to study in the future. As for the neural architecture, people have proposed many advanced versions of neural networks over simple autoencoders for under-determined image-to-image translating tasks such as Generative Adversarial Networks (GANs) \cite{karras2018progressive} and flow-based networks \cite{lugmayr2020srflow} for image super-resolution (SR) task. In general, designing a more advanced neural architecture with the minimal size for sampling map reconstruction is a promising next step. Also, it may be beneficial to switch our autoencoders to advanced reward-driven neural networks based on reinforcement learning (e.g., use screen-space \cite{huo2020adaptive} for the first bounce and revert to our proposed system for the indirect bounces).

\paragraph{Sub-voxel granularity. }
In our current system, all the intersection points in a single voxel share the same sampling map. This is not ideal since the incident radiance distribution continuously varies within the voxel. We can increase the caching density by subdividing the voxel to smaller ones, but there is always an upper limit of the available memory. One possible way to resolve this problem is to interpolate multiple reconstructed sampling maps from more than one neighboring voxels weighted by the distance in order to form a continuous-varying sampling map in space, which may need a fast implementation of the extensive image summations on GPU-based renderers. Another way is to train a neural network that can reconstruct smoothly-changing density maps for arbitrary positions in the voxel. The network can take some auxiliary features and relative positions in the voxel as additional inputs, and use them to infer how radiance field changes at the sub-voxel level. In either way, we can reduce the number of voxels in the hash grid and save a lot of memory since the density maps can continuously vary in space. Decoupling the caching from density reconstruction is an exciting topic worth to study in the future.
